Semantic Evolvement Enhanced Graph Autoencoder for Rumor Detection

Due to the rapid spread of rumors on social media, rumor detection has become an extremely important challenge. Recently, numerous rumor detection models which utilize textual information and the propagation structure of events have been proposed. However, these methods overlook the importance of semantic evolvement information of event in propagation process, which is often challenging to be truly learned in supervised training paradigms and traditional rumor detection methods. To address this issue, we propose a novel semantic evolvement enhanced Graph Autoencoder for Rumor Detection (GARD) model in this paper. The model learns semantic evolvement information of events by capturing local semantic changes and global semantic evolvement information through specific graph autoencoder and reconstruction strategies. By combining semantic evolvement information and propagation structure information, the model achieves a comprehensive understanding of event propagation and perform accurate and robust detection, while also detecting rumors earlier by capturing semantic evolvement information in the early stages. Moreover, in order to enhance the model's ability to learn the distinct patterns of rumors and non-rumors, we introduce a uniformity regularizer to further improve the model's performance. Experimental results on three public benchmark datasets confirm the superiority of our GARD method over the state-of-the-art approaches in both overall performance and early rumor detection.

==> sections/theoretical-analysis.tex <==
\section{Theoretical Understanding of Graph Masked Autoencoder}

There is a viewpoint that generative and contrastive methods adhere to different philosophies, where contrastive methods deal with the inter-data information while generative methods focus on the intra-data information~\cite{survey2021tkde}. However, we perform a deep analysis and give an insight that generative methods, such as GraphMAE, perform implicit graph contrastive learning.
In our framework, contexts with mask can be viewed as contrastive samples. 

% On the one hand, GraphMAE aligns the positive pairs in original feature space. On the other hand, the reconstructed features will not fall into the limited area in feature space as long as the masked features are not identical, but reconstruction loss cannot lead to uniformly distributed representations.
% only if the masked features are distributed uniformly.

\subsection{GraphMAE Performs Implicit Context-Level Graph Contrastive Learning}

% \subsection{$\mathcal{L}_{\mathrm{SCE}}$ is Lower Bounded by Context-Level Alignment Loss $\mathcal{L}_{\mathrm{Align}}^{\text{c}}$}


\begin{mdframed}[backgroundcolor=gray!15,hidealllines=true,innerleftmargin=2pt,innerrightmargin=2pt]
\noindent\textbf{Assumption 4.1.\label{assum4-1}} For any graph decoder $g$, we assume the existence of a pseudo-inverse graph encoder $f_g$ such that the resulting pseudo graph autoencoder $h_g = g \circ f_g$ satisfies $\mathbb{E}_x\left\|h_g(\boldsymbol{x})-\boldsymbol{x}\right\|^2 \leq \varepsilon$, where $\boldsymbol{x}$ represents the feature of masked node $v \in \widetilde{\mathcal{V}}$.
\end{mdframed}

This assumption is likely to hold in practice, since the GNN-based encoder and decoder degenerate to MLPs when input contains only one node, and MLPs already demonstrate excellent performance on the autoencoding task~\cite{autoencoding}.


\begin{mdframed}[backgroundcolor=gray!15,hidealllines=true,innerleftmargin=2pt,innerrightmargin=2pt]
\noindent\textbf{Theorem 4.2.\label{theo4-2}} Under Assumption 4.1, the SCE loss in \cref{sce} can be lower bounded by a pretext loss:
\begin{equation}
\begin{aligned}
&\mathcal{L}_{\text {SCE }}(h) \geq \frac{\gamma}{2}\mathcal{L}_{\text {Pretext }}(h)-\frac{\gamma}{2}\varepsilon+\text { const }, \\
\text { where } &\mathcal{L}_{\text {Pretext }}(h) =-\underset{{v_i \in \widetilde{\mathcal{V}}}}{\mathbb{E}} h_g\left(\boldsymbol{x}_i\right)^{\top} h\left(c_i\right).
\end{aligned}
\label{eq1}
\end{equation}
\end{mdframed}

% =-\operatorname{tr}\left(H^{\top} \bar{A}_M H_g\right),
\noindent\textbf{\textit{Proof of Theorem 4.2.}} With Assumption 4.1, and considering that the features are all normalized, we have:
% \begin{align*}
% % \begin{equation*}
% % \begin{aligned}
%     \mathcal{L}_{\mathrm{SCE}}&= \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}}\left(1- {\boldsymbol{x}_i^{\top}} h(c_i)\right)^\gamma \\
%     % &\geq 2^{\gamma-1} - 2^{\gamma-1} \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} {\boldsymbol{x}_i}^{\top} h(c_i) \\
%     &\geq \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (1 - \gamma{\boldsymbol{x}_i^{\top}} h(c_i)) \tag{Bernoulli's inequality} \\
%     % &= 2^{\gamma-1} - 2^{\gamma-1} (2 - \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2 )\\
%     &= 1 - \gamma \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \boldsymbol{x}_i^{\top} h(c_i) \\
%     &= 1 - \gamma (1 - \frac{1}{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2)) \tag{features are normalized}\\
%     &= 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2 \\
%     &= 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (\|\boldsymbol{x}_i - h(c_i)\|^2 + \varepsilon) -  \frac{\gamma }{2}\varepsilon \\
%     &\geq 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (\|\boldsymbol{x}_i - h(c_i)\|^2 + \|h_g(\boldsymbol{x}_i)-\boldsymbol{x}_i\|^2) -\frac{\gamma }{2}\varepsilon \tag{Assumption 4.1} \\
%     &\geq 1-\gamma + \frac{\gamma }{4}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|h_g(\boldsymbol{x}_i) - h(c_i)\|^2 - \frac{\gamma }{2}\varepsilon \tag{$\|a+b\|^2 \leq 2(\|a\|^2+\|b\|^2)$} \\
%     &= -\frac{\gamma }{2} \underset{{v_i \in \widetilde{\mathcal{V}}}}{\mathbb{E}} h_g\left(\boldsymbol{x}_i\right)^{\top} h\left(c_i\right) -\frac{\gamma }{2}\varepsilon + 1-\frac{\gamma }{2} \tag{features are normalized}  \\
%     &= \frac{\gamma}{2}\mathcal{L}_{\text {Pretext }}(h)-\frac{\gamma}{2}\varepsilon+\text { const }
% % \end{aligned}
% \label{sce}
% % \end{equation*}
% \end{align*}
% \begin{align*}
% % \begin{equation*}
% % \begin{aligned}
%     &\mathcal{L}_{\mathrm{SCE}}= \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}}\left(1- {\boldsymbol{x}_i^{\top}} h(c_i)\right)^\gamma \\
%     % &\geq 2^{\gamma-1} - 2^{\gamma-1} \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} {\boldsymbol{x}_i}^{\top} h(c_i) \\
%     &\geq \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (1 - \gamma{\boldsymbol{x}_i^{\top}} h(c_i)) \tag{Bernoulli's inequality} \\
%     % &= 2^{\gamma-1} - 2^{\gamma-1} (2 - \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2 )\\
%     &= 1 - \gamma \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \boldsymbol{x}_i^{\top} h(c_i) \\
%     &= 1 - \gamma (1 - \frac{1}{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2)) \tag{features are normalized}\\
%     &= 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2 \\
%     &= 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (\|\boldsymbol{x}_i - h(c_i)\|^2 + \varepsilon) -  \frac{\gamma }{2}\varepsilon \tag{Assumption 4.1}\\
%     &\geq 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (\|\boldsymbol{x}_i - h(c_i)\|^2 + \|h_g(\boldsymbol{x}_i)-\boldsymbol{x}_i\|^2) -\frac{\gamma }{2}\varepsilon.
% % \end{aligned}
% \label{sce}
% % \end{equation*}
% \end{align*}
\begin{align*}
% \begin{equation*}
% \begin{aligned}
    &\mathcal{L}_{\mathrm{SCE}}= \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}}\left(1- {\boldsymbol{x}_i^{\top}} h(c_i)\right)^\gamma \\
    % &\geq 2^{\gamma-1} - 2^{\gamma-1} \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} {\boldsymbol{x}_i}^{\top} h(c_i) \\
    &\geq \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (1 - \gamma{\boldsymbol{x}_i^{\top}} h(c_i)) \tag{Bernoulli's inequality} \\
    &= \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (1 - \gamma(1 - \frac{1}{2} \|\boldsymbol{x}_i - h(c_i)\|^2)) \tag{features are normalized} \\
    % &= 2^{\gamma-1} - 2^{\gamma-1} (2 - \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2 )\\
    % &= 1 - \gamma \underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \boldsymbol{x}_i^{\top} h(c_i) \\
    % &= 1 - \gamma (1 - \frac{1}{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2)) \tag{features are normalized}\\
    &= 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|\boldsymbol{x}_i - h(c_i)\|^2 \\
    &= 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (\|\boldsymbol{x}_i - h(c_i)\|^2 + \varepsilon) -  \frac{\gamma }{2}\varepsilon \tag{Assumption 4.1}\\
    &\geq 1-\gamma + \frac{\gamma }{2}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (\|\boldsymbol{x}_i - h(c_i)\|^2 + \|h_g(\boldsymbol{x}_i)-\boldsymbol{x}_i\|^2) -\frac{\gamma }{2}\varepsilon.
% \end{aligned}
\label{sce}
% \end{equation*}
\end{align*}

Since the inequality $\|a+b\|^2 \leq 2(\|a\|^2+\|b\|^2)$ holds, we can further obtain:
\begin{align*}
    \mathcal{L}_{\mathrm{SCE}} &\geq 1-\gamma + \frac{\gamma }{4}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} \|h_g(\boldsymbol{x}_i) - h(c_i)\|^2 - \frac{\gamma }{2}\varepsilon \\
    &= 1-\gamma + \frac{\gamma }{4}\underset{v_i \in \widetilde{\mathcal{V}}}{\mathbb{E}} (2-2h_g\left(\boldsymbol{x}_i\right)^{\top} h\left(c_i\right))) - \frac{\gamma }{2}\varepsilon \\
    &= -\frac{\gamma }{2} \underset{{v_i \in \widetilde{\mathcal{V}}}}{\mathbb{E}} h_g\left(\boldsymbol{x}_i\right)^{\top} h\left(c_i\right) -\frac{\gamma }{2}\varepsilon + 1-\frac{\gamma }{2} \\
    &= \frac{\gamma}{2}\mathcal{L}_{\text {Pretext }}(h)-\frac{\gamma}{2}\varepsilon+\text { const }.
\label{sce-2}
\end{align*}

Then we define the context-level alignment loss, which is an objective of context-level GCL, and we prove it is a lower bound of pretext loss above.
\begin{mdframed}[backgroundcolor=gray!15,hidealllines=true,innerleftmargin=2pt,innerrightmargin=2pt]
\noindent\textbf{Definition 4.3. \textit{(Context-Level Alignment Loss)}\label{def4-3}} The alignment loss for positive context pairs $(c, c^+)$ is defined as:
\begin{equation}
\mathcal{L}_{\text {Align }}^{\text{c}}(h)=-\underset{{(c, c^{+})}\sim p_{\mathrm{pos}}^c}{\mathbb{E}} h\left(c\right)^{\top} h\left(c^{+}\right).
\label{eq2}
\end{equation}
\end{mdframed}

This loss in the form of dot product and the loss in the form of mean squared error (MSE) as shown in \cref{eq:align_loss} are equivalent because the reconstructed features $\{h(c)\}_{c\in \mathcal{C}}$ are all normalized.

\begin{mdframed}[backgroundcolor=gray!15,hidealllines=true,innerleftmargin=2pt,innerrightmargin=2pt]
\noindent\textbf{Theorem 4.4.\label{theo4-4}} The pretext loss in \cref{eq1} can be lower bounded by the context-level alignment loss in \cref{eq2}:
\begin{equation}
\mathcal{L}_{\text {Pretext }}(h) \geq \frac{1}{2} \mathcal{L}_{\text {Align}}^{\text{c}}(h)+\text{const}.
\end{equation}
\end{mdframed}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{./figures/context_graph4.pdf}
    \vspace{-4pt}
    \caption{Context graph based on 2-hop connectivity in context-feature graph.}
    \label{fig:context_graph}
    \vspace{-8pt}
\end{figure}

To facilitate the proof of Theorem 4.4, we define the context-feature graph induced from the mask, as illustrated in \cref{fig:context_graph}. The context-feature graph is a bipartite graph that indicates the relations between masked node features and their contexts, which are utilized to reconstruct the masked node features. 
we use $\mathcal{F}=\{f_i\}_{i=1}^{F}$ to denote the set of node features.
For any node $v_i$ that is masked, there exists a feature node $f_j$ whose feature is equal to the feature of the masked node, i.e., $\boldsymbol{x}_i=f_j$.
Note that nodes with the same features correspond to the same feature node in our graph.
The adjacency matrix of context-feature graph is defined as $\mathbf{A}_{\mathrm{CF}}\in \mathbb{R}^{C\times F}$, where $(\mathbf{A}_{\mathrm{CF}})_{i,j}=w_{c_i,f_j}$ between $c_i \in \mathcal{C}, f_j \in \mathcal{F}$ is defined as their joint probability. In other words, there is an edge between $c_i$ and $f_j$ if and only if they belong to a complementary context-feature pair. The normalized adjacency matrix is defined as $\tilde{\mathbf{A}}_{\mathrm{CF}} = \mathbf{D}_{\mathrm{C}}^{-1/2}\mathbf{A}_{\mathrm{CF}}\mathbf{D}_{\mathrm{F}}^{-1/2}$, where $\mathbf{D}_{\mathrm{C}}, \mathbf{D}_{\mathrm{F}}$ are the diagonal degree matrices with elements $d_{c_i}=\sum_{f_j}w_{c_i,f_j}$ and $d_{f_j}=\sum_{c_i}w_{c_i,f_j}$.


\noindent\textbf{\textit{Proof of Theorem 4.4.}} With our defined context-feature graph, the $\mathcal{L}_{\text {Pretext }}(h)$ in \cref{eq1} can be reformulated as:
\begin{equation}
    \mathcal{L}_{\text {Pretext }}(h) =-\underset{{v_i \in \widetilde{\mathcal{V}}}}{\mathbb{E}} h_g\left(\boldsymbol{x}_i\right)^{\top} h\left(c_i\right) = -\tr(\mathbf{H}_g \tilde{\mathbf{A}}_{\mathrm{CF}} \mathbf{H})
\end{equation}
where $\mathbf{H}$ denotes the output matrix of $h$ on $\mathcal{C}$ whose $c_i$-th row is $\mathbf{H}_{c_i} = \sqrt{d_{c_i}}h(c_i)$, and $\mathbf{H}_g$ denotes the output matrix of $h_g$ on $\mathcal{F}$ whose $f_j$-th row is $(\mathbf{H}_g)_{f_j} = \sqrt{d_{f_j}}h_g(f_j)$.
Then, we have:
\begin{align*}
&\mathcal{L}_{\text {Pretext }}(h)  =-\tr(\mathbf{H}_g^{\top} \tilde{\mathbf{A}}_{\mathrm{CF}} \mathbf{H}) \\
& \geq-\frac{1}{2}\left(\left\|\mathbf{H}_g\right\|^2_\mathrm{F}+\left\| \tilde{\mathbf{A}}_{\mathrm{CF}}\mathbf{H}\right\|_\mathrm{F}^2\right) \tag{$\tr(\mathbf{AB}) \leq \frac{1}{2}\left(\|\mathbf{A}\|_\mathrm{F}^2+\|\mathbf{B}\|_\mathrm{F}^2\right)$}\\
& =-\frac{1}{2} \operatorname{tr}\left( \tilde{\mathbf{A}}_{\mathrm{CF}}^{\top} \tilde{\mathbf{A}}_{\mathrm{CF}}  \mathbf{H} \mathbf{H}^{\top}\right)-\frac{1}{2} \tag{$\left\|\mathbf{H}_g\right\|_\mathrm{F}^2=\sum_{f_j} d_{f_j}\left\|h_g\left(f_j\right)\right\|^2=1$} \\
& =-\frac{1}{2} \sum_{c, c^{+}} \sum_{f_j} \frac{w_{c,f_j}w_{c^{+},f_j}}{d_{f_j}} h\left(c\right)^{\top} h\left(c^{+}\right)-\frac{1}{2} \\
& =-\frac{1}{2} \sum_{c, c^{+}} (\mathbf{A}_{\mathrm{C}})_{c, c^{+}} h\left(c\right)^{\top} h\left(c^{+}\right)-\frac{1}{2} \\
& =\frac{1}{2} \mathcal{L}_{\text {align }}^{\text{c}}(h)-\frac{1}{2},
\end{align*}
where $\|\mathbf{H}\|_\mathrm{F}$ denotes the Frobenius norm of $\mathbf{H}$. Here we define $(\mathbf{A}_{\mathrm{C}})_{c, c^{+}}=\sum_{f_j} \frac{w_{c,f_j}w_{c^{+},f_j}}{d_{f_j}}$, which represents the joint probability of positive context pair $(c, c^+)$. As shown in \cref{fig:context_graph}, we construct the homogeneous context graph based on the 2-hop connectivity from the context-node bipartite graph. The edge weights represent the probability of forming positive pairs between contexts. In this case, $\mathbf{A}_{\mathrm{C}} \in \mathbb{R}^{C\times C}$ represents the adjacency matrix of this context graph.



Combining Theorem 4.2 and Theorem 4.4, we arrive at the main theorem showing that GraphMAE’s node-level reconstruction loss can be bounded by the alignment loss of the positive context pairs drawn according to the masked nodes.

\begin{mdframed}[backgroundcolor=gray!15,hidealllines=true,innerleftmargin=2pt,innerrightmargin=2pt]
\noindent\textbf{Theorem 4.5.\label{theo4-5}} Under Assumption 4.1, GraphMAE’s nodel-level reconstruction loss in \cref{sce} can be lower bounded by the context-level alignment loss in \cref{eq2}:
\begin{equation}
\begin{aligned}
   \mathcal{L}_{\text{SCE}}(h) &\geq \frac{\gamma}{4} \mathcal{L}_{\text {Align}}^{\text{c}}(h)-\frac{\gamma}{2}\varepsilon+\text{const}\\
&=-\frac{\gamma}{4} \underset{{c, c^{+}}}{\mathbb{E}} h\left(c\right)^{\top} h\left(c^{+}\right)-\frac{\gamma}{2}\varepsilon+\text{const}. 
\end{aligned}
\label{conclustion}
\end{equation}
\end{mdframed}

Following Theorem 4.5, a small GraphMAE's reconstruction loss implies a small context-level alignment loss, which indicates that GraphMAE implicitly aligns the representations of contexts.


% Note that the implicit GCL is performed in original feature space, but latent space. 
% However, based on \cite{U-MAE}, GraphMAE loss can be lower bounded by an alignment loss in the output space. Moreover, we can show that GraphMAE loss is further lower bounded by an alignment loss in the latent space, which indicates that GraphMAE has the capability to align positive pairs in the latent space.

% If we introduce AU loss in original feature space, the alignment loss is invalid because it is induced from reconstruction loss, while the uniformity loss would violate the reconstruction loss. If we introduce AU loss in latent space, The alignment loss may not be helpful for reconstruction, as it neglects the role of the graph structure in the input to the decoder.
% Thus, we cannot directly introduce unsupervised alignment loss and uniformity loss.
\vspace{4pt}
\noindent\textbf{Intuitive explanation.} Here, we provide an intuitive explanation for our theoretical result. We reiterate that GraphMAE employs the autoencoder to reconstruct the masked node features based on the contexts of these mask nodes. When two (or more) masked nodes have the same or very similar features, then their contexts have the same reconstruction goal, and thus these contexts will be encoded as similar latent representations. In the paradigm of contrastive learning, these contexts can be considered as positive pairs.

\vspace{-8pt}

\subsection{Limitations of GraphMAE\label{subsection:limitation}}
The theoretical analysis above builds a bridge between GraphMAE and GCL. Despite the lack of understanding of GraphMAE, GCL has been thoroughly studied by numerous works. Therefore, we can identify the limitations of GraphMAE with the well-established tools in GCL. Specifically, we further discuss the limitations of GraphMAE from the perspective of alignment and uniformity.
% , which have been considered as two key properties of high-quality representations in contrastive learning.

% Although GraphMAE has the capability to align positive pairs in the latent space, the effect of alignment is restricted by the quality of positive pairs generated by the masking operation. We observe that the uniform random masking strategy adopted by GraphMAE cannot provide enough information about hard-to-align pairs.

% In addition, although GraphMAE can avoid the full feature collapse, but cannot ensure the uniformity of learned representations.


For alignment, although GraphMAE is proven to have the ability to align positive pairs, we point out that the practical alignment effect not only depends on the model's ability, but also influenced by the masking strategy. Concretely, the optimization objective is computed as an expectation over the distribution of mask, so the optimal solution is affected by this distribution. 
% We then discuss the implications of the distribution in different objectives. For reconstruction loss in \cref{sce}, the distribution is about the mask, while for alignment loss in \cref{eq2}, it is the distribution of the positive pairs. In the implicit GCL performed by GraphMAE, the positive pairs are also induced from mask. 
% Thus, it is essentially the distribution of the mask that affects the alignment effect. 
% No matter the reconstruction loss in \cref{sce} or the alignment loss in \cref{eq2}, it is essentially the distribution of the mask that affects the effect of alignment.
Further, the uniform random masking strategy adopted by GraphMAE ignores the imbalanced distribution of easy and hard samples, and cannot provide enough information about hard-to-align pairs. 
% Therefore, the random masking strategy limits the effect of alignment. 

For uniformity, we point out that representation uniformity is not strictly guaranteed in GraphMAE. 
% The reconstructed features will not fall into the same point in feature space as long as the masked features are not identical, but reconstruction loss cannot lead to uniformly distributed representations.
Specifically, GraphMAE avoids full feature collapse, i.e., the learned representations do not collapse to a fixed point in the feature space, as long as the masked features are not identical. However, reconstruction loss cannot lead to uniformly distributed representations. In \cref{fig:pilot}, we observe that the representations still suffer from dimensional collapse, i.e., the representation is not uniformly distributed in the feature space. Therefore, the representation uniformity can also be improved.

In a nutshell, we summarize the following limitations of GraphMAE in terms of alignment and uniformity:
\begin{itemize}
    \item \textbf{Alignment performance is still restricted by the distribution of mask, which is decided by the masking strategy.}
    \item \textbf{Uniformity performance is not strictly guaranteed.}
\end{itemize}
